Multi-Scale Representation Learning on Proteins

Proteins are fundamental biological entities mediating key roles in cellular function and disease. This paper introduces a multi-scale graph construction of a protein -- HoloProt -- connecting surface to structure and sequence. The surface captures coarser details of the protein, while sequence as primary component and structure -- comprising secondary and tertiary components -- capture finer details. Our graph encoder then learns a multi-scale representation by allowing each level to integrate the encoding from level(s) below with the graph at that level. We test the learned representation on different tasks, (i.) ligand binding affinity (regression), and (ii.) protein function prediction (classification). On the regression task, contrary to previous methods, our model performs consistently and reliably across different dataset splits, outperforming all baselines on most splits. On the classification task, it achieves a performance close to the top-performing model while using 10x fewer parameters. To improve the memory efficiency of our construction, we segment the multiplex protein surface manifold into molecular superpixels and substitute the surface with these superpixels at little to no performance loss.

==> content/checklist.tex <==
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{The main claims made in the abstract can be verified by the results presented in Table~\ref{tab:res_pdbbind} and~\ref{tab:res_enzyme}.}
  \item Did you describe the limitations of your work?
    \answerYes{See Section~\ref{sec:limitations}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{
    Our work is relevant to scientific disciplines aiming at learning with proteins. By integrating the multi-scale nature of proteins, we expect our method to be more robust and have fewer unforeseen side-effects than previous methods. However, proteins and their interaction with other molecules are highly complex and results might be strongly influenced by the experimental setting. Thus, results of any protein representation method have to be taken with care, and need further evaluation. We show this remaining inaccuracy in Section~\ref{sec:evaluation}.
    Hence, while potential misuse can never be ruled out, our presented method predominantly promises positive societal and scientific impact.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{We provide code, datasets and installation instructions via an external URL.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{The dataset splits, hyperparameters are described in Appendix~\ref{app:datasets} and \ref{app:hyperparams}}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{We report our results according to the standards of related work as mean accuracy, mean RMSE, Pearson or Spearman correlation with corresponding standard deviation.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{We report the types of resources used as well as the total computation time in Appendix~\ref{app:computing}.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{Our method is based on open-source libraries which we credit in Appendix~\ref{app:exp_details}.}
  \item Did you mention the license of the assets?
    \answerYes{We mention the license of used assets in Appendix~\ref{app:exp_details}.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{We include new assets via an external URL.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{The used datasets are publicly available and shared via licensed described in Appendix~\ref{app:datasets}.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{The datasets do not include personally identifiable information and offensive content.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> content/trash.tex <==
\begin{table}[t]
\caption[Ligand Binding Affinity Prediction]{\textbf{Protein-Ligand Binding Affinity Prediction} Comparison of the prediction of ligand binding affinity using the PDBbind dataset \citep{liu2017} of \textsc{HoloProt} against other methods. Results are reported for 3 runs.}
    \label{tab:res_pdbbind}
    \centering
    \begin{adjustbox}{max width=.9\linewidth}
    \begin{tabular}{lcccc}
    \toprule
    \textbf{Model} & \textbf{\# Params} &  \multicolumn{3}{c}{\textbf{Scaffold}} \\ \\
    & & RMSE & Pearson & Spearman \\
    \cmidrule{3-5}
    \citet{ozturk2018} & 1.93 M & 1.908 $\pm$ 0.145 & 0.384 $\pm$ 0.014 & 0.387 $\pm$ 0.016\\
    \citet{bepler2019} & 48.8 M & 1.864 $\pm$ 0.009 & 0.269 $\pm$ 0.002 & 0.285 $\pm$ 0.019\\
    \citet{tape2019} & 93.0 M & 1.680 $\pm$ 0.055 & 0.487 $\pm$ 0.029 & 0.462 $\pm$ 0.051 \\
    \citet{gainza2020} & 0.62 M & 1.583 $\pm$ 0.132 & 0.416 $\pm$ 0.111 & 0.412 $\pm$ 0.126 \\
    \citet{townshend2020}\footnotemark[1] & - & - & - & - \\
    \citet{townshend2020}\footnotemark[2] & - & - & - & - \\
    \citet{hermosilla2021} & 5.80 M & 1.592 $\pm$ 0.012 & 0.365 $\pm$ 0.024 & 0.373 $\pm$ 0.019 \\
    \\
    \textsc{HoloProt} (\colcircle{lightblue}) & 1.44 M & 1.523 $\pm$ 0.028 & 0.489 $\pm$ 0.019 & 0.491 $\pm$ 0.020\\
    \textsc{HoloProt} (\coldiamond{darkblue}) & 1.76 M & \textbf{1.516} $\pm$ \textbf{0.014} & \textbf{0.491} $\pm$ \textbf{0.016} & \textbf{0.493} $\pm$ \textbf{0.014} \\ \\
    \end{tabular}
    \end{adjustbox}
\end{table}
\begin{table}
    \vspace{-1.5em}
    \centering
    \begin{adjustbox}{max width=\linewidth}
    \begin{tabular}{ccccccccc}
    \toprule
    \multicolumn{3}{c}{\textbf{Sequence Identity (30 \%)}} & &  \multicolumn{3}{c}{\textbf{Sequence Identity (60 \%)}} \\ \\
    
    RMSE & Pearson & Spearman & & RMSE & Pearson & Spearman \\
    \cmidrule{1-3}\cmidrule{5-7}
    1.866 $\pm$ 0.080 & 0.472 $\pm$ 0.022 & 0.471 $\pm$ 0.024 && 1.762 $\pm$ 0.261 & 0.666 $\pm$ 0.012 & 0.663 $\pm$ 0.015\\
    1.985 $\pm$ 0.006	& 0.165 $\pm$ 0.006	& 0.152 $\pm$ 0.024 && 1.891 $\pm$ 0.004 & 0.249 $\pm$ 0.006 & 0.275 $\pm$ 0.008 \\
    1.890 $\pm$ 0.035 & 0.338 $\pm$ 0.044 & 0.286 $\pm$ 0.124 && 1.633 $\pm$ 0.016 & 0.568 $\pm$ 0.033 & 0.571 $\pm$ 0.021 \\
    1.484 $\pm$ 0.018 & 0.467 $\pm$ 0.020 & 0.455 $\pm$ 0.014 && 1.426 $\pm$ 0.017 & 0.709 $\pm$ 0.008 & 0.701 $\pm$ 0.011 \\
    \textbf{1.429} $\pm$ \textbf{0.042} & 0.541 $\pm$ 0.029 & 0.532 $\pm$ 0.033 && 1.450 $\pm$ 0.024 & 0.716 $\pm$ 0.008 & 0.714 $\pm$ 0.009 \\
    1.936 $\pm$ 0.120 & \textbf{0.581} $\pm$ \textbf{0.039} & \textbf{0.647} $\pm$ \textbf{0.071} && 1.493 $\pm$ 0.010 & 0.669 $\pm$ 0.013 & 0.691 $\pm$ 0.010 \\
    1.554 $\pm$ 0.016 & 0.414 $\pm$ 0.053 & 0.428 $\pm$ 0.032 && 1.473 $\pm$ 0.024 & 0.667 $\pm$ 0.011 & 0.675 $\pm$ 0.019 \\
    \\
    1.464 $\pm$ 0.006 & 0.509 $\pm$ 0.002 & 0.500 $\pm$ 0.005 && \textbf{1.365} $\pm$ \textbf{0.038} & \textbf{0.749} $\pm$ \textbf{0.014} & \textbf{0.742} $\pm$ \textbf{0.011} \\
    1.491 $\pm$ 0.004 & 0.491 $\pm$ 0.014 & 0.482 $\pm$ 0.017 && 1.416 $\pm$ 0.022 & 0.724 $\pm$ 0.011 & 0.7152 $\pm$ 0.006 \\
    \bottomrule \\
    \multicolumn{4}{c}{\large \colcircle{lightblue} \enspace full surface  \hfill \coldiamond{darkblue} \enspace molecular superpixels}
    \end{tabular}
    \end{adjustbox}
\end{table}
